Self-Recovering Sensor-Actor Networks

Wireless sensor-actor networks are a recent development of wireless networks where both ordinary sensor nodes and more sophisticated and powerful nodes, called actors, are present. In this paper we formalize a recently introduced algorithm that recovers failed actor communication links via the existing sensor infrastructure. We prove via refinement that the recovery is terminating in a finite number of steps and is distributed, thus self-performed by the actors. Most importantly, we prove that the recovery can be done at different levels, via different types of links, such as direct actor links or indirect links between the actors, in the latter case reusing the wireless infrastructure of sensors. This leads to identifying coordination classes, e.g., for delegating the most security sensitive coordination to the direct actor-actor coordination links, the least real-time constrained coordination to indirect links, and the safety critical coordination to both direct actor links and indirect sensor paths between actors. Our formalization is done using the theorem prover in the RODIN platform.

==> eptcsdata.tex <==
\providecommand{\firstpage}{47}
\providecommand{\publicationstatus}{M.R. Mousavi and G. Sala{\"u}n (Ed.): International
Workshop \\ on the  Foundations of Coordination Languages and \\ Software Architectures (FOCLASA 2010).\\
EPTCS 30, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.30.4}{10.4204/EPTCS.30.4}}
\pdfoutput=1

